Cross-Language Approach for Quranic QA

Question answering systems face critical limitations in languages with limited resources and scarce data, making the development of robust models especially challenging. The Quranic QA system holds significant importance as it facilitates a deeper understanding of the Quran, a Holy text for over a billion people worldwide. However, these systems face unique challenges, including the linguistic disparity between questions written in Modern Standard Arabic and answers found in Quranic verses written in Classical Arabic, and the small size of existing datasets, which further restricts model performance. To address these challenges, we adopt a cross-language approach by (1) Dataset Augmentation: expanding and enriching the dataset through machine translation to convert Arabic questions into English, paraphrasing questions to create linguistic diversity, and retrieving answers from an English translation of the Quran to align with multilingual training requirements; and (2) Language Model Fine-Tuning: utilizing pre-trained models such as BERT-Medium, RoBERTa-Base, DeBERTa-v3-Base, ELECTRA-Large, Flan-T5, Bloom, and Falcon to address the specific requirements of Quranic QA. Experimental results demonstrate that this cross-language approach significantly improves model performance, with RoBERTa-Base achieving the highest MAP@10 (0.34) and MRR (0.52), while DeBERTa-v3-Base excels in Recall@10 (0.50) and Precision@10 (0.24). These findings underscore the effectiveness of cross-language strategies in overcoming linguistic barriers and advancing Quranic QA systems

==> sections/architecture_diagram.tex <==
\tikzstyle{process} = [rectangle, rounded corners, minimum width=2.5cm, minimum height=1cm, text centered, draw=black, fill=blue!20, font=\small]
\tikzstyle{data} = [rectangle, minimum width=2.5cm, minimum height=1cm, text centered, draw=black, fill=red!20, font=\small]
\tikzstyle{circlebox} = [circle, minimum width=1cm, minimum height=1cm, text centered, draw=black, fill=green!20, font=\small]
\tikzstyle{arrow} = [thick, ->, >=stealth]

\begin{figure}[ht]
    \centering
    \begin{tikzpicture}[node distance=0.5cm, every node/.style={scale=0.8}] % Reduced spacing and scaled nodes

    % Q-Text
    \node (qText) [data, text centered] {Q-Text};

    % Positive documents
    \node (posDocsLabel) [text centered, below=0.4cm of qText, xshift=-1.5cm, font=\small] {Positive passages};
    \node (posDocs) [draw, rectangle, minimum width=2.5cm, minimum height=1.2cm, below=0.3cm of posDocsLabel, font=\small] {
        \begin{tabular}{l|c}
        \textbf{Text} & \textbf{Relevance} \\ \hline
        Passage1 & 1 \\
        Passage3 & 1 \\
        ... & 1
        \end{tabular}
    };

    % Negative documents
    \node (negDocsLabel) [text centered, right=1cm of posDocsLabel, font=\small] {Negative passages};
    \node (negDocs) [draw, rectangle, minimum width=2.5cm, minimum height=1.2cm, below=0.3cm of negDocsLabel, font=\small] {
        \begin{tabular}{l|c}
        \textbf{Text} & \textbf{Relevance} \\ \hline
        Passage6 & 0 \\
        Passage14 & 0 \\
        ... & 0
        \end{tabular}
    };

    % Randomizer
    \node (randomizer) [process, below=0.5cm of posDocs, xshift=1.5cm] {Randomizer};

    % Combined data
    \node (combinedLabel) [below=0.4cm of randomizer, font=\small] {Combined Data for each question};
    \node (combined) [draw, rectangle, minimum width=3cm, minimum height=1.5cm, below=0.3cm of combinedLabel, font=\small] {
        \begin{tabular}{l|c}
        \textbf{Text} & \textbf{Relevance} \\ \hline
        Passage3 & 1 \\
        Passage6 & 0 \\
        ... & ...
        \end{tabular}
    };

    % LM using Cross-Encoder
    \node (lm) [process, right =0.5cm of combined] {LLM \& LM using Cross-Encoder};

    % LM Output
    \node (embedding) [process, right=0.4cm of lm] {LLM \& LM Output};
    % Retrieval
    \node (retrieval) [process, above=0.8cm of embedding] {Retrieval};
    % Test Cases
    \node (testCases) [data, above=0.8cm of retrieval] {Test Cases};



    % Answers
    \node (answersLabel) [right=0.9cm of testCases, font=\small] {Answers};
    \node (answers) [draw, rectangle, minimum width=2.5cm, minimum height=1.2cm, below=0.3cm of answersLabel, font=\small] {
        \begin{tabular}{l}
        Passage2 \\
        Passage5 \\
        Passage9 \\
        ...
        \end{tabular}
    };

    % Arrows
    \draw [arrow] (qText) -- (posDocsLabel);
    \draw [arrow] (qText) -- (negDocsLabel);
    \draw [arrow] (posDocs) -- (randomizer);
    \draw [arrow] (negDocs) -- (randomizer);
    \draw [arrow] (randomizer) -- (combined);
    \draw [arrow] (combined) -- (lm);
    \draw [arrow] (lm) -- (embedding);
    \draw [arrow] (embedding) -- (retrieval);
    \draw [arrow] (retrieval) -- (answers);
    \draw [arrow] (testCases) -- (retrieval); % Arrow connecting testCases to retrieval

    \end{tikzpicture}
    \caption{Workflow for LLM \& LM training}
    \label{fig:lm_workflow}
\end{figure}
